Scalable Planning in Multi-Agent MDPs

Multi-agent Markov Decision Processes (MMDPs) arise in a variety of applications including target tracking, control of multi-robot swarms, and multiplayer games. A key challenge in MMDPs occurs when the state and action spaces grow exponentially in the number of agents, making computation of an optimal policy computationally intractable for medium- to large-scale problems. One property that has been exploited to mitigate this complexity is transition independence, in which each agent's transition probabilities are independent of the states and actions of other agents. Transition independence enables factorization of the MMDP and computation of local agent policies but does not hold for arbitrary MMDPs. In this paper, we propose an approximate transition dependence property, called $\delta$-transition dependence and develop a metric for quantifying how far an MMDP deviates from transition independence. Our definition of $\delta$-transition dependence recovers transition independence as a special case when $\delta$ is zero. We develop a polynomial time algorithm in the number of agents that achieves a provable bound on the global optimum when the reward functions are monotone increasing and submodular in the agent actions. We evaluate our approach on two case studies, namely, multi-robot control and multi-agent patrolling example.

==> Analysis.tex <==
\section{Optimality Analysis}
\label{sec:optimality}
%This section considers the optimality of our proposed approach. %We first analyze the optimality guarantees for an $\epsilon$-TI MDP. We then characterize the parameter $\epsilon$. Then, we analyze the complexity of our approach.

%\subsection{Optimality of Algorithm}
%\label{subsec:optimality}
We analyze the optimality in three stages. First, we define a TI-MDP, and prove that the policies returned by our algorithm are within a provable bound of a local optimum of the TI-MDP. We then use submodularity of the reward function to prove that the local optimal policies provide a constant-factor approximation to the global optimum on the TI-MDP. Finally, we prove that the approximate global optimum on the TI-MDP is also an approximate global optimum for the original MDP.

{\color{red}
We define $\hat{\pi} = \{\hat{\pi}_{1},\ldots,\hat{\pi}_{m}\}$ to be the policy returned by our algorithm. Let $\hat{q}$ be the joint stationary distribution of the agents in the MDP $\mathcal{M}$ arising from these policies. We construct a TI-MDP $\hat{\mathcal{M}} = (S, A, \hat{P}, \hat{R})$. The transition function $\hat{P}$ is defined by $$\hat{P}(s,a,s^{\prime}) = \prod_{i=1}^{m}{\hat{P}_{i}(s_{i},a_{i},s_{i}^{\prime})}.$$ The reward function $\hat{R} = R(s,a)$. We observe that, by construction, if $\mathcal{M}_{i}$ is the local MDP obtained at the last iteration of Algorithm \ref{algo:Stack}, then $J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) = J_{\hat{\mathcal{M}}}(\hat{\pi})$ for all $i$. 

\begin{lemma}
\label{lemma:TI-MDP-local-opt}
The policy $\hat{\pi}$ returned by Algorithm \ref{algo:Stack} is a $1/(1+\delta)$-local optimum for MDP $\hat{\mathcal{M}}$.
\end{lemma}

\emph{Proof:} By construction, the algorithm terminates if, for all $i$, there is no policy $\pi_{i}$ such that $$J_{\hat{\mathcal{M}}}(\pi_{i}, \hat{\pi}_{-i}) = J_{\mathcal{M}_{i}}(\pi_{i}) \geq (1+\delta)J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) = (1+\delta)J_{\hat{\mathcal{M}}}(\hat{\pi}),$$ implying that $\hat{\pi}$ is a $1/(1+\delta)$-local optimum of $\hat{\mathcal{M}}$.

Based on the local optimality, we can derive the following optimality bound for $\hat{\pi}$.
\begin{lemma}
\label{lemma:TI-MDP-optimality}
Let $\pi^{\ast}$ denote the optimal local policies for MDP $\mathcal{M}$. Then $$J_{\hat{\mathcal{M}}}(\hat{\pi}) \geq \frac{1}{2+\delta m}J_{\hat{\mathcal{M}}}(\pi^{\ast}).$$
\end{lemma}

\emph{Proof:} The proof follows from the submodularity of $J_{\hat{\mathcal{M}}}$ (Proposition \ref{prop:submodular-TI}) and Lemma \ref{lemma:local-opt-submodular-matroid}.

Lemma \ref{lemma:TI-MDP-optimality} provides an optimality bound with respect to the TI-MDP $\hat{\mathcal{M}}$. Next, we leverage the $\epsilon$-TI property to derive an optimality bound with respect to the given MDP $\mathcal{M}$. We start with the following  preliminary results.

\begin{lemma}
\label{lemma:total-variation-bound}
For any state $s$ and policy $\pi$, $||P(s,\pi,\cdot)-\overline{P}(s,\pi,\cdot)||_{TV} \leq m\epsilon$, where $P$ and $\overline{P}$ are the transition matrices corresponding to $\mathcal{M}$ and $\hat{\mathcal{M}}$, respectively.
\end{lemma}

A proof can be found in the technical appendix. We next exploit the bound in Lemma \ref{lemma:total-variation-bound} to approximate the gap between the $J_{\mathcal{M}}$ and $J_{\hat{\mathcal{M}}}$.

\begin{lemma}
\label{lemma:MDP-approximation}
Suppose that $\mathcal{M}$ is $\epsilon$-TI MDP. Define $\phi = \frac{R_{max}}{R_{min}}2m\epsilon\overline{\lambda}$.  For any policy $\pi$, $J_{\hat{\mathcal{M}}}(\pi) \geq (1-\phi)J_{\mathcal{M}}(\pi)$ and $J_{\mathcal{M}}(\pi) \geq (1-\phi)J_{\hat{\mathcal{M}}}(\pi)$.
\end{lemma}

\emph{Proof:} Let $q_{\mathcal{M}}$ and $q_{\hat{\mathcal{M}}}$ denote the stationary distributions induced by policy $\pi$ on MDPs $\mathcal{M}$ and $\hat{\mathcal{M}}$. We have $$|J_{\hat{\mathcal{M}}}(\pi)-J_{\mathcal{M}}(\pi)| \leq R_{max} ||q_{\mathcal{M}}-q_{\hat{\mathcal{M}}}||_{1}.$$ By Lemma \ref{lemma:perturbation}, $$||q_{\mathcal{M}}-q_{\hat{\mathcal{M}}}||_{1} \leq 2\overline{\lambda}m\epsilon.$$ Rearranging terms gives the desired result.

Combining these derivations gives the following.

\begin{theorem}
\label{theorem:optimality-bound}
Let $\mathcal{M}$ be an $\epsilon$-TI MDP and $\hat{\pi}$ and $\pi^{\ast}$ denote the output of Algorithm \ref{algo:Stack} and the optimal policies, respectively. Then $$J_{\mathcal{M}}(\hat{\pi}) \geq \frac{1}{2+m\delta}(1-\phi)^{2}J_{\mathcal{M}}(\pi^{\ast}).$$
\end{theorem}

\emph{Proof:} We have 
\begin{eqnarray*}
J_{\mathcal{M}}(\hat{\pi}) &\geq& (1-\phi)J_{\hat{\mathcal{M}}}(\hat{\pi}) \geq \frac{1}{2+m\delta}(1-\phi)J_{\hat{\mathcal{M}}}(\pi^{\ast}) \\
&\geq & \frac{1}{2+m\delta}(1-\phi)^{2}J_{\hat{\mathcal{M}}}(\pi^{\ast}),
\end{eqnarray*}
where the first inequality follows from Lemma \ref{lemma:MDP-approximation}, the second inequality follows from Lemma \ref{lemma:TI-MDP-optimality}, and the third inequality follows from Lemma \ref{lemma:MDP-approximation}.
}
%and $\hat{q}$ to be the joint stationary distribution of the agent states arising from these policies. The induced TI-MDP $\hat{\mathcal{M}} = (\hat{S}, \hat{A}, \hat{P}, \hat{R})$ is constructed from the MDP $\mathcal{M} = (S, A, P, R)$ as follows. The state and action spaces are identical, i.e., $\hat{S} = S$ and $\hat{A} = A$. The transition probabilities $\hat{P}_{i}$ of each agent are given by 
%\begin{multline}
%    \label{eq:equiv-TI-transition}
%\hat{P}_{i}(s_{i},a_{i},s_{i}^{\prime}) = \sum_{s_{-i},s_{-i}^{\prime}}{\hat{q}(s_{-i}|s_{i})}\\
%\cdot P(\{s_{i},s_{-i}\}, \{a_{i},a_{-i}\},\{s_{i}^{\prime},s_{-i}^{\prime}\}).
%\end{multline}
%The rewards are defined by $\hat{R}(s,a) = R(s,a)$. We observe that by construction $J_{\mathcal{M}}(\hat{\pi}) = J_{\hat{\mathcal{M}}}(\hat{\pi})$, i.e., the rewards of the policy $\hat{\pi}$ are the same in the MDPs $\mathcal{M}$ and $\hat{\mathcal{M}}$.

%We denote a policy $\pi$ to be locally optimal with respect to MDP $\mathcal{M}$ if for every $i$ and every local policy $\tilde{\pi}_{i}$, we have $J_{\mathcal{M}}(\pi) \geq J_{\mathcal{M}}(\tilde{\pi}_{i},\pi_{-i})$. A policy $\pi$ is $\theta$-locally optimal if for every $i$ and every local policy $\tilde{\pi}_{i}$, we have $(1+\theta)J_{\mathcal{M}}(\pi) \geq J_{\mathcal{M}}(\tilde{\pi}_{i},\pi_{-i})$.

%\begin{lemma}
%\label{lemma:optimality-1}
%Suppose that $\mathcal{M}$ is an $\epsilon$-TI MDP.  Define $\overline{\epsilon} = \frac{\epsilon R_{max}}{R_{min}}\overline{\lambda}$. Then the policy $\hat{\pi}$ returned by our algorithm is a $\left(\frac{1-\overline{\epsilon}}{(1+\delta)(1+\overline{\epsilon})}\right)$-local optimal policy for the TI-MDP $\mathcal{M}$.
%\end{lemma}

%\emph{Proof:} We define two MDPs $\mathcal{M}_{i}$ and $\hat{\mathcal{M}}_{i}$. The MDP $\hat{\mathcal{M}}_{i}$ is the local MDP of agent $i$ at the last iteration of our algorithm. The MDP $\mathcal{M}_{i}$ has state space $S_{i}$, action space $A_{i}$, transition function $\hat{P}_{i}$ as in (\ref{eq:equiv-TI-transition}), and reward function $$\hat{R}_{i}(s_{i},a_{i}) = \sum_{s_{-i}}{\hat{q}(s_{-i}|s_{i})R(\{s_{i},s_{-i}\}, \{a_{i}, \pi_{-i}(s_{-i})\})}.$$ By construction, under policy $\hat{\pi}_{i}$, the stationary probability of state $s_{i} \in S_{i}$ in $\hat{\mathcal{M}}_{i}$ is equal to $\hat{q}(s_{i})$. Hence 
%\begin{eqnarray}
%J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) &=& \sum_{s_{i}}{\hat{q}(s_{i})R_{i}(s_{i},\hat{\pi}_{i}(s_{i}))} \\
%&=& \sum_{s_{i}}{\hat{q}(s_{i})\sum_{s_{-i}}{\hat{q}(s_{-i}|s_{i})}} \\
%\nonumber 
%&& \cdot R(\{s_{i},s_{-i}\},\{\hat{\pi}_{i}(s_{i}),\hat{\pi}_{-i}(s_{-i})\}) \\
%\label{eq:local-opt-2}
%&=& \sum_{s}{\hat{q}(s)R(s,\hat{\pi}(s))} = J_{\hat{\mathcal{M}}}(\hat{\pi})
%\end{eqnarray}

%Hence the average reward from choosing policy $\hat{\pi}_{i}$ in local MDP $\mathcal{M}_{i}$ is equal to the reward from choosing policy $\hat{\pi}$ in the TI-MDP $\hat{\mathcal{M}}$. We next show that 
%\begin{equation}
 %   \label{eq:local-opt-1}
  %  (1-\overline{\epsilon})J_{\hat{\mathcal{M}}_{i}}(\hat{\pi}_{i}) \leq J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) \leq (1+\overline{\epsilon})J_{\hat{\mathcal{M}}_{i}}(\hat{\pi}_{i}).
%\end{equation}
%We have that 
%\begin{eqnarray*}
%J_{\hat{\mathcal{M}}_{i}}(\hat{\pi}_{i}) &=& \sum_{s_{i}}{q_{\mathcal{M}_{i}}(s_{i})R_{\mathcal{M}_{i}}(s_{i},\hat{\pi}_{i}(s_{i}))} \\ J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) &=& \sum_{s_{i}}{q_{\hat{\mathcal{M}}_{i}}(s_{i})R_{\mathcal{M}_{i}}(s_{i},\hat{\pi}_{i}(s_{i}))}, 
%\end{eqnarray*}
%where $q_{\mathcal{M}_{i}}$ and $q_{\hat{\mathcal{M}}_{i}}$ are the stationary distributions of agent $i$'s state under policy $\hat{\pi}_{i}$ in the MDPs $\mathcal{M}_{i}$ and $\hat{\mathcal{M}}_{i}$, respectively.  
%Taking the difference between these quantities, we have $$|J_{\tilde{\mathcal{M}}_{i}}(\hat{\pi}_{i})-J_{\mathcal{M}_{i}}(\hat{\pi}_{i})| \leq R_{max}||q_{\mathcal{M}_{i}}-q_{\hat{\mathcal{M}}_{i}}||_{1}$$ via Holder's inequality. The stationary distributions  satisfy $$||q_{\mathcal{M}_{i}}-q_{\tilde{\mathcal{M}}_{i}}||_{1} \leq \epsilon\overline{\lambda}$$ by Lemma \ref{lemma:perturbation}. Hence (\ref{eq:local-opt-1}) holds. Combining (\ref{eq:local-opt-2}) and (\ref{eq:local-opt-1}), we obtain 
%\begin{equation*}
%(1+\overline{\epsilon})J_{\tilde{\mathcal{M}}}(\hat{\pi}) = (1+\overline{\epsilon})J_{\tilde{\mathcal{M}}_{i}}(\hat{\pi}_{i}) \geq J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) 
%\end{equation*}
%By construction of the algorithm, we have $(1+\delta)J_{\mathcal{M}_{i}}(\hat{\pi}) \geq J_{\mathcal{M}_{i}}(\tilde{\pi}_{i})$ for any policy $\tilde{\pi}_{i}$, and thus 
%\begin{eqnarray*}
%(1+\delta)J_{\mathcal{M}_{i}}(\hat{\pi}_{i}) &\geq& J_{\mathcal{M}_{i}}(\tilde{\pi}_{i}) \geq (1-\overline{\epsilon})J_{\mathcal{M}_{i}}(\tilde{\pi}_{i}) \\
%&=& (1-\overline{\epsilon})J_{\mathcal{M}}(\hat{\pi}_{-i},\tilde{\pi}_{i}).
%\end{eqnarray*}
%Combining these inequalities gives the desired result. %$\qed$

%Lemma \ref{lemma:optimality-1} implies that the policy $\hat{\pi}$ is an approximate local optimum for the  TI-MDP $\hat{\mathcal{M}}$. The following result implies that $\hat{\pi}$ is within a  bound of the global optimum for $\hat{\mathcal{M}}$. 

%\begin{proposition}
%\label{prop:local-MDP-submodular}
%Let $\pi^{\ast}$ denote the optimal solution to (\ref{eq:combinatorial-form}). Then 
%\begin{equation}
%    \label{eq:local-MDP-submodular}
%    J_{\hat{\mathcal{M}}}(\hat{\pi}) \geq \frac{1}{2+\theta m}J_{\hat{\mathcal{M}}}(\pi^{\ast}).
%\end{equation}
%where $\theta = \frac{1-\overline{\epsilon}}{(1+\delta)(1+\overline{\epsilon})}$.
%\end{proposition}

%\emph{Proof:} By Proposition \ref{prop:submodular-TI}, $J_{\tilde{\mathcal{M}}}(\pi)$ is submodular as a function of $\pi$. By Lemma \ref{lemma:local-opt-submodular-matroid}, any $\theta$-local optimum of $J_{\hat{\mathcal{M}}}$ is a $\frac{1}{2+\theta m}$-approximation of the optimal solution. In particular, (\ref{eq:local-MDP-submodular}) holds.



%Next, we will bound the reward $J_{\hat{\mathcal{M}}}(\pi^{\ast})$ under the optimal policy $\pi^{\ast}$ in comparison with the true reward $J_{\mathcal{M}}(\pi^{\ast})$. We have the following preliminary result.
%\begin{lemma}
%\label{lemma:total-variation-bound}
%For any state $s$ and policy $\pi$, $||P(s,\pi,\cdot)-\overline{P}(s,\pi,\cdot)||_{TV} \leq m\epsilon$, where $P$ and $\overline{P}$ are the transition matrices corresponding to $\mathcal{M}$ and $\hat{\mathcal{M}}$, respectively.
%\end{lemma}


%The proof can be found in the technical appendix. We are now ready to state the second local optimality result.

%\end{IEEEeqnarray*}
%\begin{proposition}
%\label{prop:local-opt-2}
%For the optimal policy $\pi^{\ast}$, we have $J_{\tilde{\mathcal{M}}}(\pi^{\ast}) \geq (1-\phi) J_{\mathcal{M}}(\pi^{\ast})$, where $$\phi = \frac{R_{max}}{R_{min}}2m\epsilon\Lambda_{1}((I-P(\pi^{\ast}))^{\#}.$$
%\end{proposition}

%\emph{Proof:} We have that 
%\begin{eqnarray*}
%|J_{\hat{\mathcal{M}}}(\pi^{\ast})-J_{\mathcal{M}}(\pi^{\ast})| &=& |\sum_{s \in S}{(\hat{q}(s)-q(s))R(s,\pi(s))}| \\
%&\leq& R_{max}||\hat{q}(s)-q(s)||_{1}.
%\end{eqnarray*}
%It remains to bound $||\tilde{q}(s)-q(s)||_{1}$. Define $\hat{P}$ as the transition matrix of $\hat{\mathcal{M}}$ under policy $\pi^{\ast}$ and $P$ as the transition matrix of $\mathcal{M}$ under policy $\pi^{\ast}$. Our approach is to bound $||\hat{P}-P||_{1}$ and then apply Lemma \ref{lemma:perturbation}. By Lemma \ref{lemma:total-variation-bound}, we have $||\hat{P}-P||_{1} \leq 2m\epsilon$, yielding the desired result. %For any $s$, we develop a bound for $\sum_{s^{\prime}}{|\hat{A}(s,s^{\prime})-A(s,s^{\prime})|}$ via the coupling method. We let $X$ denote a random variable over $S$ with distribution $\tilde{P}(s,\cdot)$ and $Y$ a random variable over $S$ with distribution $P(s,\cdot)$. From Lemma \ref{lemma:coupling}, we have $$||\hat{A}(s,\cdot) - A(s,\cdot)||_{TV} \leq \frac{1}{2}Pr(X \neq Y).$$ Furthermore, we have that 
%\begin{eqnarray*}
%Pr(X \neq Y) &=& Pr(s^{\prime} \neq s^{\prime\prime}) = %Pr\left(\bigcup_{i=1}^{m}{s_{i}^{\prime} \neq s_{i}^{\prime\prime}}\right) \\
%&\leq& \sum_{i=1}^{m}{Pr(s_{i}^{\prime} \neq s_{i}^{\prime\prime})} \leq m\epsilon
%\end{eqnarray*}
%completing the proof.

%The following result summarizes the optimality bounds of our algorithm.

%\begin{theorem}
%\label{theorem:optimality}
%For an $\epsilon$-TI MDP with maximum and minimum rewards $R_{max}$ and $R_{min}$, our proposed algorithm returns a policy $\hat{\pi}$ satisfying $$J_{\mathcal{M}}(\hat{\pi}) \geq \frac{1}{2+\theta m}\left(1-\frac{R_{max}}{R_{min}}2m\epsilon \overline{\lambda}\right)J_{\mathcal{M}}(\pi^{\ast}) $$ where $\theta = \frac{1-\overline{\epsilon}}{(1+\delta)(1+\overline{\epsilon})}$ and $\overline{\epsilon} = \frac{\epsilon R_{max}}{R_{min}}\overline{\lambda}$ 
%\end{theorem}

%\emph{Proof:} From Proposition \ref{prop:local-MDP-submodular}, we have $$J_{\mathcal{M}}(\hat{\pi}) = J_{\hat{\mathcal{M}}}(\hat{\pi}) \geq \frac{1}{2+\theta m}J_{\hat{\mathcal{M}}}(\pi^{\ast}).$$ Furthermore, by Proposition \ref{prop:local-opt-2}, $$J_{\tilde{\mathcal{M}}}(\pi^{\ast}) \geq \left(1-\frac{R_{max}}{R_{min}}2m\epsilon\bar{\lambda}\right) J_{\mathcal{M}}(\pi^{\ast}).$$ Combining these inequalities yields the desired result. 

==> Simulation-v2.tex <==
\section{Simulation}\label{sec:simulation}
% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Agents, Targets \\Number} & \thead{Grid\\ Size} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ & \thead{Avg. Run Time of\\ Algorithm \ref{algo:Stack}}\\
%     \hline
%   2, 1& $3 \times 3$ & 81 & 16 & 0.345 & 0.345 & 0.347 & 0.351& 0.351 & 0.351 & 26.47s\\
%   \hline
%   2, 2 & $3 \times 3$ & 81 & 16 & 0.441 & 0.440 & 0.439 & 0.443& 0.443 & 0.443 & 28.13s\\
%     \hline
%   2, 1 & $4 \times 4$ &256& 16  & 0.235 & 0.237 & 0.237 & 0.238  &0.238 & 0.238 & 56.00s\\
%     \hline
%     2, 2 & $4 \times 4$& 256 & 16 & 0.322 & 0.322 & 0.322 &0.328 & 0.328 & 0.328 & 75.33s\\
%     \hline
%     2, 1 & $5 \times 5$ & 625& 16 & 0.190 & 0.191 & 0.189 & 0.191 & 0.191 & 0.191 & 462.10s\\
%     \hline
%     3, 1 & $3 \times 3$ & 729 & 64 & 0.431  & 0.476 & 0.528 & 0.457 &  0.499 & 0.543  & 1754.84s \\
%     \hline
%     3, 1 & $4 \times 4$ & 4096  & 64 & 0.293 & 0.336  & 0.331 & 0.341 & 0.341 & 0.341 & 3178.86s\\
%     \hline
%     4, 1 & $2 \times 2$ & 256 & 256 & 0.621 & 0.660 & 0.752 & 0.634 &  0.670 & 0.761 & 586.64s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and average run time achieved using our proposed approach for different multi-agent robot control settings for three different dependency parameters ($\epsilon$ = $0.5$, $0.9$ and $0.1$). Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}. } 
% \label{table:robot}
% \end{table*}

\begin{table*}[t!]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
     \multicolumn{6}{|c|}{MDP Setting} & \multicolumn{3}{|c|}{Average Reward } & \multicolumn{3}{|c|}{Run Time (seconds)} \\
    \hline
    \thead{Number of Agents\\ and Targets $(N,B)$} & \thead{Grid Size\\ $L$}  & Target Location & \thead{Agents' Initial\\ Locations}&  \thead{State Space\\ Size} & \thead{Action Space\\ Size} &Algorithm \ref{algo:Stack} & \thead{Global MDP\\ Approach} & Ratio & Algorithm \ref{algo:Stack} & \thead{Global MDP\\ Approach} & Ratio \\
    \hline
  2, 1& $3 \times 3$ & 6 & (0,2) & 81 & 16 & 0.312 & 0.333 & 93.69\% & 0.246& 0.142 & 173.2\% \\
  \hline
  2, 2 & $5 \times 5$ & (20,24) & (3,5) & 625 & 16 & 0.268 & 0.269 & 99.63\% & 3.08 & 3.01 & 102.3\% \\
    \hline
  3, 1 & $3 \times 3$ & 6 & (0,0,2) & 729 & 64  & 0.460 & 0.504 & 91.27\% & 6.51  & 24.1 & 27.01\%\\
    \hline
    3, 1 & $3 \times 3$ & 8 & (1,1,2) & 729 & 64  & 0.435 & 0.475 & 91.58\% & 6.66  & 25.2 & 26.43\%\\
    \hline
    3, 1 & $4 \times 4$ & 15 & (0,0,3) & 4096 & 64 & 0.318 & 0.334 & 95.21\% & 41.9 & 446 & 9.395\%\\
    \hline
     3, 1 & $4 \times 4$ & 12 & (1,1,2) & 4096 & 64 & 0.337 & 0.355 & 94.93\% & 41.9 & 439 & 9.544\%\\ 
    \hline
    4, 1 & $2 \times 2$ & 3 & (0,0,1,1) & 256 & 256 & 0.758 & 0.766  & 98.96\% & 4.76 & 35.7 & 13.33\% \\
    \hline
    2, 2 & $10 \times 10$ & (90,99) & (0,9) & 10000 & 16 & 0.125 & 0.125 & 100\% & 56.9 &  451 & 12.62\% \\
    \hline
    2, 2 & $10 \times 10$ & (55,77) & (5,99) & 10000 & 16 & 0.241 & 0.241 & 100\% & 56.8 &  429 & 13.24\% \\
    \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of average reward and run time when Multi-robot control problem is solved using Algorithm \ref{algo:Stack} versus using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox} on corresponding global MDP ($\mathcal{M}$). Both appraches are compared under different sizes of grids $L$, number of agents $N$, number of targets $B$, and initial locations of the agents. The `Ratio' of average reward in Table \ref{table:robot} is obtained as the average reward of Algorithm \ref{algo:Stack} divided by that of the global MDP approach. The `Ratio' of run time in Table \ref{table:robot} is obtained as the run time incurred by Algorithm \ref{algo:Stack} divided by that of the global MDP approach.} 
\label{table:robot}
\end{table*}



In this section, we present our simulation results. We consider two scenarios, namely, multi-robot control and a multi-agent patrolling example. Both simulations are implemented using Python 3.8.5 on a workstation with Intel(R) Xeon(R) W-2145 CPU @ 3.70GHz processor and $128$~GB memory. Given the transition and reward matrices, an MDP is solved using \textit{Python MDP Toolbox} \cite{MDPtoolbox}. 

\subsection{Multi-robot Control}
\subsubsection{Simulation Settings}
We consider a set of $N > 1$ robots whose goal is to cover maximum number of targets from a set of fixed targets $B$ positioned in a $L \times L$ grid environment. Robots initially start from a fixed set of grid locations. At each time $t = 1, 2, \ldots$, each robot $i$ can move one grid position horizontally or vertically from the current grid position by taking some action $a_i\in A_i := \{left, down, right, up\}$. For each robot $i$, let $D_i := \{d(a_i)\}_{a_i \in A_i}$ denotes the set of grid positions that can be reached from the current grid position $s_i$ under each action $a_i \in A_i$. $d(a_i)$ is the grid position corresponds to $(s_i, a_i)$. Note that $d(a_i) = \varnothing$, if $a_i$ is not a valid action (e.g., $a_i \in \{left, down\}$ at the bottom left corner of the grid are not valid actions). Let $P_i$ be the transition probability function associated with robot $i$ and $P_i(s_i, a_i, s_i')$ be the probability of robot $i$ transitions from a grid position $s_i$ to $s_i'$ under action $a_i$. Let $n(s_i')$ be the number of robots at $s_i'$ after taking actions $(a_i, a_{-i})$. Then,
\begin{equation*}
    P_i(s_i,a_i,s_i')=\begin{cases}
    c,~\mbox{if $s_i' = d(a_i)$ and $n(s_i') < K$}\\
    \frac{1-c}{|D_i|-1},\mbox{if $s_i' \in D_i \setminus d(a_i)$ and $n(s_i') < K$}\\
    \epsilon c,~\mbox{if $s_i' = d(a_i)$ and $n(s_i') \geq K$}\\
    \frac{1-\epsilon c}{|D_i|-1},\mbox{if $s_i' \in D_i \setminus d(a_i)$ and $n(s_i') \geq K$}\\
    0,~\mbox{otherwise, }
    \end{cases}
\end{equation*}
where $K \geq 1$. Uncertainty in the environment is modeled by the parameter $0 \leq c \leq 1$ and the  transition dependencies between the robots are modeled by the parameter $0 \leq \epsilon\ \leq 1$.

%Particularly, when there are $K>0$ robots target at the same grid position, we say transition dependency occurs. The transition probability to the target location of each robot that incurs transition dependency scales down by a factor $0<\epsilon\leq 1$. To summarize, the transition probability from a grid position $s_i$ to a target grid position $s_i'$ by taking action $a_i$ is given as

% Hence, when a robot takes an action $a_i$ to reach a grid position $s_i$ (e.g., move up by one grid position), it will only reach its desired grid position with $0 <c<1$ probability. With remaining probability $1-c$, the robot will reach other neighbouring vertical or horizontal grid position in $D(s_i)$. The transition noise parameter $c$ ensures that the induced Markov chain is irreducible, and thus the average reward maximization problem is well-posed \cite{bertsekas1995dynamic}. When there are more than $K>0$ robots target at the same grid position, we say transition dependency occurs, and the transition probability of reaching the target grid position for each of these robots becomes $\epsilon c$, where $0 < \epsilon \leq  1$. Parameter $\epsilon$ captures the $\epsilon$-TI property among the agents. For each agent $i$, the transition probability from a grid position $s_i$ to a target grid position $s_i'$ by taking action $a_i$ is given as
% \begin{equation*}
%     P_i(s_i,a_i,s_i')=\begin{cases}
%     c,~\mbox{ if agent $i$ targets at $s_i'$ and }\\
%     \quad\quad\quad\quad\mbox{no transition dependency occurs}\\
%     \frac{1-c}{|D|-1},~\mbox{if agent $i$ does not target at $s_i'$}\\
%     \quad\quad\mbox{and no transition dependency occurs}\\
%     \epsilon c,~\mbox{ if agent $i$ targets at $s_i'$ and}\\
%     \quad\quad\quad\quad\mbox{transition dependency occurs}\\
%     \frac{1-\epsilon c}{|D|-1},~\mbox{ if agent $i$ does not target at $s_i'$}\\
%     \quad\quad\quad\mbox{and transition dependency occurs}
%     \end{cases}
% \end{equation*}

We model the multi-robot control problem as an MDP $\mathcal{M} = (S, A, P, R)$. The state space $S = S_1 \times \ldots \times S_N$, where $S_i=\{0, \ldots, L^2-1\}$ for all $i=1,\ldots,N$. The action space $A = A_1 \times \ldots \times A_N$, where $A_i=\{left,down,right,up\}$ is the action space of agent $i$. The transition probability matrix is denoted as $P$. The probability of transitioning from a state $s=(s_1,\ldots,s_N)\in S$ to some target state $s'=(s_1',\ldots,s_N')\in S$ by taking action $a=(a_1,\ldots,a_m)\in A$ is given as $P(s,a,s')=\prod_{i=1}^mP_i(s_i,a_i,s_i')$. The \textit{submodular} reward $R$ of $\mathcal{M}$ is given by $R(s_{t},\pi(s_{t}))= \sum_{b \in B}(1-(1-\eta)^{N_b})$, where $N_b$ is the number of robots visiting target $b$ following a joint policy $\pi(s_{t})$ at a state state $s_{t}$. The parameter $\eta$ captures the effectiveness of having $N_b$ agents at target $b$. Similar \textit{submodular} reward has been used in \cite{kumar2017decentralized}.


%  The parameter $\epsilon$ in this problem setting defines the transition dependency in the transition probability matrix $P$ of $\mathcal{M}$. Specifically, when $\epsilon \rightarrow 1$, the transition dependency among agents becomes weaker, and MDP $\mathcal{M}$ approaches TI-MDP. Hence, this formulation defines an $\epsilon$-TI MDP $\mathcal{M}$.

\begin{table*}[t!]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
     \multicolumn{4}{|c|}{MDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Run Time (seconds)}  \\
    \hline
    \thead{Defender, Adversary\\Number} & \thead{Location\\ Number} & \thead{State Space\\ Size} & \thead{Defenders' Action \\Space Size} &Algorithm \ref{algo:Stack} & \thead{Global MDP\\Approach} &Ratio &Algorithm \ref{algo:Stack} & \thead{Global MDP\\Approach} &Ratio \\
    \hline
   2,1& 3 & 27 & 9 & 0.774 & 0.775 & 99.87\% & 0.133 & 0.435 & 30.57\% \\
   \hline
   3,1 & 3 & 81 & 27 & 0.865 & 0.866 & 99.88\% & 1.93 & 6.49 & 29.73\% \\
    \hline
   3,2 & 3 & 243 & 27  & 1.73 & 1.73 & 100\% & 22.84  & 157 & 14.54\% \\
    \hline
    2,1 & 5 & 125 & 25 & 0.768 & 0.768 & 100\% & 5.56 & 18.13 & 30.67\% \\
    \hline
    3,1 & 5 & 625& 125 & 0.856 & 0.856 & 100\% & 239 &  2823 & 8.466\% \\
    \hline
    2,1 & 7 & 343& 49 & 0.766 & 0.766 & 100\% & 68.7 &  358 & 19.19\% \\
    \hline
    2,1 & 8 & 512& 64 & 0.766 & 0.766 & 100\% & 188 & 1295 & 14.52\% \\
    \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of average reward and run time when Multi-Agent Security game is solved using Algorithm \ref{algo:Stack} versus using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox} on corresponding global MDP ($\mathcal{M}$). Both approaches are compared under different  number of defenders, adversaries, and locations. The `Ratio' of average reward in Table \ref{table:robot} is obtained as the average reward of Algorithm \ref{algo:Stack} divided by that of the global MDP approach. The `Ratio' of run time in Table \ref{table:robot} is obtained as the run time incurred by Algorithm \ref{algo:Stack} divided by that of the global MDP approach.} 
\label{table:security}
\end{table*}






\subsubsection{Simulation Results}

We use Algorithm~\ref{algo:Stack} to find a set of policies for the robots that maximizes their average reward. Parameters $\delta$, $K$, $\eta$, and $\beta$ are set to $0$, $1$, $0.75$ and $0.9$, respectively. The transition probability for each agent is calculated by evaluating \eqref{eq:algo-local-transition-function} over $\lfloor\frac{N*L*L}{2}\rfloor$ samples of actions $\{a_i,\Bar{a}_{-i}\}$ and states $\{s_{i}',\Bar{s}_{-i}'\}$. We test Algorithm \ref{algo:Stack} under different sizes of grids $L$, number of agents $N$, number of targets $B$, and initial locations of the agents. For each setting, we execute Algorithm \ref{algo:Stack} for $100$ trials, and take the average over the trials as the performance of Algorithm~\ref{algo:Stack}. We compare Algorithm \ref{algo:Stack} with the a global MDP approach, which calculates the optimal values using relative value iteration algorithm \cite{bertsekas1995dynamic} provided by \textit{Python MDP Toolbox} \cite{MDPtoolbox} on MDP $\mathcal{M}$. Note that the state space of MDP $\mathcal{M}$ is exponential in grid size $L$ and number of agents $N$. The action space is exponential in $N$. The total size of all local MDPs for all agents constructed using \eqref{eq:algo-local-transition-function} and \eqref{eq:algo-local-reward} grows linearly with respect to the number of agents. As the number of agents and/or grid size of examples increase, the global MDP approach incurs a heavy memory computation overhead to the system. For an example, when $2$ robots trying to reach $1$ target in a $10 \times 10$ grid, it requires around $1.29$~Gb of memory to compute the solution using global MDP approach, while our proposed approach only requires $1.45$~Mb memory to calculate the policy. Therefore, the global MDP approach is not computationally efficient for larger example sizes.

Table \ref{table:robot} shows the simulation results obtained using Algorithm \ref{algo:Stack} and the global MDP approach. We observe that our proposed approach provides more than $90\%$ optimality with respect to the average reward achieved by the agents for all settings, while incuring comparable run time when the example size is small and much less run time when the example sizes increase. Particularly, as the number of agents and the grid size increase, e.g., two agents, two targets, and $10\times 10$ grid, our proposed approach maintains more than $100\%$ optimality with only $12.62\%$ run time, compared with the global MDP approach. Hence, our proposed approach shows scalability to mutli-agent scenarios with $\epsilon$-TI property.

% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Agents, Targets \\Number} & \thead{Grid\\ Size} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\eta=0.1$ & $\eta=0.5$ &$\eta = 0.9$ & $\eta=0.1$ & $\eta=0.5$ & $\eta=0.9$ & \thead{Avg. Run Time of\\ Algorithm \ref{algo:Stack}}\\
%     \hline
%   2, 1& $3 \times 3$ & 81 & 16 & 0.345 & 0.345 & 0.347 & 0.351& 0.351 & 0.351 & 26.47s\\
%   \hline
%   2, 2 & $3 \times 3$ & 81 & 16 & 0.441 & 0.440 & 0.439 & 0.443& 0.443 & 0.443 & 28.13s\\
%     \hline
%   2, 1 & $4 \times 4$ &256& 16  & 0.235 & 0.237 & 0.237 & 0.238  &0.238 & 0.238 & 56.00s\\
%     \hline
%     2, 2 & $4 \times 4$& 256 & 16 & 0.322 & 0.322 & 0.322 &0.328 & 0.328 & 0.328 & 75.33s\\
%     \hline
%     2, 1 & $5 \times 5$ & 625& 16 & 0.190 & 0.191 & 0.189 & 0.191 & 0.191 & 0.191 & 462.10s\\
%     \hline
%     3, 1 & $3 \times 3$ & 729 & 64 & 0.431  & 0.476 & 0.528 & 0.457 &  0.499 & 0.543  & 1754.84s \\
%     \hline
%     3, 1 & $4 \times 4$ & 4096  & 64 &  &  &  & &  & & \\
%     \hline
%     4, 1 & $2 \times 2$ & 256 & 256 & 0.621 & 0.660 & 0.752 & 0.634 &  0.670 & 0.761 & 586.64s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and average run time achieved using our proposed approach for different multi-agent robot control settings for three different dependency parameters ($\eta$ = $0.5$, $0.9$ and $0.1$). Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}. } 
% \label{table:robot}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Defender, Adversary\\Number} & \thead{Location\\ Number} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ & \thead{Avg. Run Time \\of Algorithm \ref{algo:Stack}}\\
%     \hline
%   2,1& 3 & 27 & 27 & 0.563 & 0.563 & 0.563 & 0.563 & 0.563 & 0.563 & 10.7s\\
%   \hline
%   3,1 & 3 & 81 & 81 & 0.75 & 0.75 & 0.75 & 0.75& 0.75 & 0.75 & 105.5s\\
%     \hline
%   3,2 & 3 & 243 & 243  & 1.5 & 1.5 & 1.5 & 1.5  & 1.5 & 1.5 & 3092.31s\\
%     \hline
%     2,1 & 5 & 125 & 125 & 0.245 & 0.230 & 0.246 &0.46875 & 0.46875 & 0.46875 & 330.73s\\
%     \hline
%     3,1 & 5 & 625& 625 & 0.46 & 0.46 & 0.46 & 0.5625 &  0.5625& 0.5625 & 6803.3s\\
%     \hline
%     2,1 & 7 & 343& 343 & 0.29 & 0.29 & 0.29 & 0.4375 &  0.4375& 0.459 & 1080.66s\\
%     \hline
%     2,1 & 8 & 512& 512 & 0.18 & 0.18 & 0.18 & 0.428 & 0.428 & 0.428 & 4871.71s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and run time achieved using our proposed approach for different multi-agent security game settings with different dependency parameters $\epsilon$ ($\epsilon=0.1$, $0.5$ and $0.9$). The parameters $\eta$ and $\beta$ are set to $0.75$ and $0.5$, respectively. Parameters $c$ and $d$ are set as $c=d=1$. Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}.} %Table \ref{table:robot} also gives the run time incurred when computing the stationary distribution using the Monte Carlo simulation and the solver time incurred to solve for the optimal policy of each agent. \textbf{Please ignore the numbers in this Table for now.}}
% \label{table:security}
% \end{table*}


\subsection{Multi-Agent Patrolling Example}
\subsubsection{Simulation Settings}
We implement our proposed approach on a patrolling example with multiple patrol units tracking multiple moving objects among a finite set of locations $L$ as an evaluation. At each time, each patrol unit can be deployed at some location $l\in L$.

The objective of the patrol units is to compute a policy to patrol the locations to track the moving objects. Each object is assumed to follow a non-deterministic dynamics as follows. If there exists no defender that protects the adversary's target location $l$, then with probability $d$ the adversary intrudes location $l$ and with probability $(1-d)/(L-1)$ the adversary intrudes some other location $l'\neq l$. If the adversary's target location $l$ is under the protection of some defender, then with probability $\beta d$ the adversary intrudes location $l$, and with probability $(1-\beta d)/(L-1)$ the adversary intrudes some other location $l'\neq l$. This heuristic policy is assumed to be known to the defender.

The security game is modeled by an MDP $\mathcal{M}=(S,A,P,R)$, where $S=(\times_iS_i)\times(\times_jS_j)$ is the set of joint locations of the defenders and adversaries, with $S_i=L$ is the set of locations at which defender $i$ deploys its resource and $S_j=L$ is the set of locations where the adversary $j$ can intrude. The action of each defender and adversary is $A_i=A_j=L$. Thus the joint action space $A=(\times_iA_i)\times(\times_jA_j)$. We shall remark that the joint action space is defined as the Cartesian product of the action spaces of all defenders and adversaries so that we can accurately capture the transition probabilities of all defenders and adversaries. We solve the problem by optimizing over the joint action space of all the defenders, since the policies of the adversaries are known to the defender. For each defender $i$ and adversary $j$, we let
\begin{align*}
    &P_i(s_i, a_i,s_i') =\begin{cases}
    c&\mbox{ if } a_i=s_i', \not\exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \frac{1-c}{|L|}&\mbox{ if }a_i\neq s_i',\not\exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \epsilon c&\mbox{ if } a_i=s_i', \exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \frac{1-\epsilon c}{|L|}&\mbox{ if } a_i\neq s_i', \exists i'\neq i \text{ s.t. }a_{i}=a_{i'}
    \end{cases}\\
    &P_j(s_j, a_j,s_j') =\begin{cases}
    d&\mbox{ if } a_j=s_j', \not\exists i \text{ s.t. }a_{i}=a_{j'}\\
    \frac{1-d}{|L|}&\mbox{ if }a_j\neq s_j', \not\exists i \text{ s.t. }a_{i}=a_{j'}\\
    \beta d&\mbox{ if } a_j=s_j', \exists i \text{ s.t. }a_{i}=a_{j'}\\
    \frac{1-\beta d}{|L|}&\mbox{ if } a_j\neq s_j',\exists i \text{ s.t. }a_{i}=a_{j'}
    \end{cases}
\end{align*}
Here parameters $c,d\in[0,1]$ capture the transition uncertainties \cite{jiang2013game}, parameter $\epsilon\in[0,1]$ captures the transition dependency between the defenders, and $\beta\in[0,1]$ captures the adversary's reaction to the defenders' actions. Let $s=(\times_is_i)\times(\times_js_j)$ and $s'=(\times_is'_i)\times(\times_js'_j)$ be two joint locations. Then $P(s,a,s')=\prod_{i,j}P_i(s_i,a_i,s_i')P_j(s_j,a_j,s_j')$, where $a=(\times_is_i)\times(\times_js_j)$. We define the reward function $R(s,a)$ for each $s\in S$ and $a\in A$ as $R(s,a)=\sum_{s'\in S}r(s,a,s')P(s,a,s')$, where $r(s,a,s')=\sum_{l\in L}(1-(1-\eta)^{k_l})x_l$, where $\eta\in(0,1]$ is the effectiveness parameter, $k$ and $x$ are the number of defenders and adversaries that are in location $l$ corresponding to $s'$, respectively.



% Given the current  location $s$, each defender $i$ computes its policy $\pi_i:S\mapsto L$ to determine the next location where its resource will be deployed. Each adversary $j$ determines its next location by following policy $\tau_j:S\mapsto L$. We assume that the policy of each adversary $j$ is known to the defenders. 

\subsubsection{Simulation Results}

We use Algorithm \ref{algo:Stack} to compute the policies for the defenders, given the heuristic policies of the adversaries. Parameters $c$, $d$, $\epsilon$, $\beta$, and $\eta$ are set as $0.9$, $1$, $0.9$, $0.9$, and $0.75$, respectively. We calculate the transition probability of each defender $i$ by evaluating \eqref{eq:algo-local-transition-function} over all possible actions $(\times_{-i}a_{-i})\times(\times_{j}a_{j})$ and all possible states $(\times_{-i}s_{-i})\times(\times_{j}s_{j})$ of all adversaries and all the other defenders except $i$. We implement our proposed approach under various settings by varying the number of defenders, adversaries, and locations. For each setting, we run Algorithm \ref{algo:Stack} for $100$ trials and take the average over the trials as its performance. We compare Algorithm \ref{algo:Stack} with the global MDP approach that implements relative value iteration algorithm on MDP $\mathcal{M}$.

Table \ref{table:security} shows the simulation results obtained using Algorithm \ref{algo:Stack} and the global MDP approach. We observe that our proposed approach achieves more than $99\%$ of optimality with respect to the average reward, while incuring at most $30.57\%$ of run time over all settings. By comparing the first row, 4-th row, 6-th row, and 7-th row in Table \ref{table:security}, we have that the run time advantage provided by our proposed approach remains when we increase the number of locations. By comparing the first three rows in Table \ref{table:security}, we observe that our proposed approach remains close to optimal average reward (more than $99\%$), but scales better when the number of agents including defender and adversary increases. 



==> Simulation.tex <==
\section{Simulation}
% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Agents, Targets \\Number} & \thead{Grid\\ Size} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ & \thead{Avg. Run Time of\\ Algorithm \ref{algo:Stack}}\\
%     \hline
%   2, 1& $3 \times 3$ & 81 & 16 & 0.345 & 0.345 & 0.347 & 0.351& 0.351 & 0.351 & 26.47s\\
%   \hline
%   2, 2 & $3 \times 3$ & 81 & 16 & 0.441 & 0.440 & 0.439 & 0.443& 0.443 & 0.443 & 28.13s\\
%     \hline
%   2, 1 & $4 \times 4$ &256& 16  & 0.235 & 0.237 & 0.237 & 0.238  &0.238 & 0.238 & 56.00s\\
%     \hline
%     2, 2 & $4 \times 4$& 256 & 16 & 0.322 & 0.322 & 0.322 &0.328 & 0.328 & 0.328 & 75.33s\\
%     \hline
%     2, 1 & $5 \times 5$ & 625& 16 & 0.190 & 0.191 & 0.189 & 0.191 & 0.191 & 0.191 & 462.10s\\
%     \hline
%     3, 1 & $3 \times 3$ & 729 & 64 & 0.431  & 0.476 & 0.528 & 0.457 &  0.499 & 0.543  & 1754.84s \\
%     \hline
%     3, 1 & $4 \times 4$ & 4096  & 64 & 0.293 & 0.336  & 0.331 & 0.341 & 0.341 & 0.341 & 3178.86s\\
%     \hline
%     4, 1 & $2 \times 2$ & 256 & 256 & 0.621 & 0.660 & 0.752 & 0.634 &  0.670 & 0.761 & 586.64s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and average run time achieved using our proposed approach for different multi-agent robot control settings for three different dependency parameters ($\epsilon$ = $0.5$, $0.9$ and $0.1$). Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}. } 
% \label{table:robot}
% \end{table*}

\begin{table*}[t!]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
     \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward of Algorithm \ref{algo:Stack}} & \multicolumn{3}{|c|}{Average Reward of MDP Toolbox} \\
    \hline
    \thead{Number of Agents\\ and Targets $(N,B)$} & \thead{Grid Size\\ $L$} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ \\
    \hline
  2, 1& $3 \times 3$ & 81 & 16 & 0.345 & 0.345 & 0.347 & 0.351& 0.351 & 0.351 \\
  \hline
  2, 2 & $3 \times 3$ & 81 & 16 & 0.441 & 0.440 & 0.439 & 0.443& 0.443 & 0.443 \\
    \hline
  2, 1 & $4 \times 4$ &256& 16  & 0.235 & 0.237 & 0.237 & 0.238  &0.238 & 0.238\\
    \hline
    2, 2 & $4 \times 4$& 256 & 16 & 0.322 & 0.322 & 0.322 &0.328 & 0.328 & 0.328 \\
    \hline
    2, 1 & $5 \times 5$ & 625& 16 & 0.190 & 0.191 & 0.189 & 0.191 & 0.191 & 0.191 \\
    \hline
    3, 1 & $3 \times 3$ & 729 & 64 & 0.431  & 0.476 & 0.528 & 0.457 &  0.499 & 0.543   \\
    \hline
    3, 1 & $4 \times 4$ & 4096  & 64 & 0.293 & 0.336  & 0.331 & 0.341 & 0.341 & 0.341 \\
    \hline
    4, 1 & $2 \times 2$ & 256 & 256 & 0.621 & 0.660 & 0.752 & 0.634 &  0.670 & 0.761 \\
    \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of average reward computed using Algorithm \ref{algo:Stack} and relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}, under different sizes of grids $L$, number of agents $N$, number of targets $B$, and transition dependency parameter $\epsilon$ ($\epsilon=0.1,0.5$ and $0.9$). Transition dependency parameter $\epsilon$ characterizes the maximum change in the probability distribution of any agent due to changes in the states and actions of the other agents. Parameter $\delta$ is set to $0$ in Algorithm \ref{algo:Stack}.} 
\label{table:robot}
\end{table*}


\label{sec:simulation}
In this section, we present our simulation results. We consider two scenarios, namely, multi-robot control and a multi-agent security game. Both simulations are implemented using Python 3.8.5 on a workstation with Intel(R) Xeon(R) W-2145 CPU @ 3.70GHz processor and $128$~GB memory. Given the transition and reward matrices, an MDP is solved using \textit{Python MDP Toolbox} \cite{MDPtoolbox}. 

%Due to exponential problem size and transition dependency, it is infeasible to create and store the transition probability matrix of the Markov Chain (MC) induced by a given policies of robots. Therefore, exact computation of stationary probability distribution $q(\cdot)$ using matrix multiplication or eigen-decomposition is infeasible in both simulations. 
In our simulations, we compute the stationary distributions of the agent states as follows. 
Given a joint policy of the agents we simulate the induced Markov chain starting from the initial state to find the number of times each state is visited. We simulate the transitions of agents starting from each state by randomly drawing an action at each state according to the joint policy. We use this frequency distribution over the joint state space to approximate $q(\cdot)$. We make sure that the induced Markov chain of the MMDP in our examples are irreducible to guarantee the existence of average reward. Moreover, we randomly initialize the simulations of Markov chain after fixed time to ensure that each state is visited often to achieve a close approximation of $q(\cdot)$ in less time. At each iteration of Algorithm \ref{algo:Stack}, we evaluate the average reward $J(\pi_i',\pi_{-i})$ (line 9 of Algorithm \ref{algo:Stack}) by simulating the policy on the induced Markov chain.
%In Algorithm \ref{algo:Stack}, the transition probability matrix and reward for each agent $i$ is also computed via simulating the Markov chain induced by the updated joint policy $\pi_{-i}$ of the other agents. 

\subsection{Multi-robot Control}
\subsubsection{Simulation Settings}
We consider a set of $N > 1$ robots whose goal is to cover maximum number of targets from a set of fixed targets $B$ positioned in a $L \times L$ grid environment. Robots initially start from a fixed set of grid locations. At each time $t = 1, 2, \ldots, $ each robot moves one grid position horizontally or vertically from the current grid position.  We assume environment is noisy. Hence, when a robot takes an action to reach a grid position (e.g., move up by one grid position), it will only reach its desired grid position with $0 <\beta<1$ probability. With remaining probability $1-\beta$, robot will reach other neighbouring vertical or horizontal grid position. We assume a set of robots reach a same grid position with $0 < \epsilon \leq  1$ probability if the number of robots trying to reach the same grid position exceeds $K >0$. 

We model the multi-robot control problem as an MMDP $\mathcal{M} = (S, A, P, R)$. State space is in the form of $S = S_1 \times \ldots \times S_N$, where each $S_i \in \{0, \ldots, L^2-1\}$. Action space has the structure of $A = A_1 \times \ldots \times A_N$, where each $A_i \in \{left, down, right, up\}$. Note that the state space of multi-robot control problem $\mathcal{M}$ is exponential in grid size $L$ and number of agents $N$. The action space is exponential in $N$.

The parameter $\epsilon$ in this problem setting defines the transition dependency in the transition structure $P$ of $\mathcal{M}$. Specifically, when $\epsilon \rightarrow 1$, the underlying $\mathcal{M}$ becomes closer to a transition independent $\mathcal{M}$. Hence, this formulation defines an $\epsilon$-transition independent $\mathcal{M}$. The \textit{submodular} reward $R$ of $\mathcal{M}$ is given by $R(s_{t},\pi(s_{t}))= \sum_{b \in B}(1-(1-\eta)^{N_b})$, where $N_b$ is the number of robots visiting target $b$ following a joint policy $\pi(s_{t})$ at a state state $s_{t}$. The parameter $\eta$ captures the effectiveness of having $N_b$ agents at target $b$. Similar type of \textit{submodular} rewards has been used in the simulations of  \cite{kumar2017decentralized}.

\begin{table*}[t!]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
     \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward of Algorithm \ref{algo:Stack}} & \multicolumn{3}{|c|}{Average Reward of MDP Toolbox}  \\
    \hline
    \thead{Defender, Adversary\\Number} & \thead{Location\\ Number} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ \\
    \hline
   2,1& 3 & 27 & 27 & 0.53 & 0.53 & 0.53 & 0.563 & 0.563 & 0.563 \\
   \hline
   3,1 & 3 & 81 & 81 & 0.75 & 0.75 & 0.75 & 0.75& 0.75 & 0.75 \\
    \hline
   3,2 & 3 & 243 & 243  & 1.5 & 1.5 & 1.5 & 1.5  & 1.5 & 1.5 \\
    \hline
    2,1 & 5 & 125 & 125 & 0.245 & 0.230 & 0.246 &0.469 & 0.469 & 0.469 \\
    \hline
    3,1 & 5 & 625& 625 & 0.46 & 0.46 & 0.46 & 0.563 &  0.563& 0.563 \\
    \hline
    2,1 & 7 & 343& 343 & 0.29 & 0.29 & 0.29 & 0.438 &  0.438& 0.459 \\
    \hline
    2,1 & 8 & 512& 512 & 0.18 & 0.18 & 0.18 & 0.428 & 0.428 & 0.428 \\
    \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of average reward computed using Algorithm \ref{algo:Stack} and relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}, when varying the number of defenders, adversaries, locations, and transition dependency parameter $\epsilon$ ($\epsilon=0.1$, $0.5$ and $0.9$). Transition dependency parameter $\epsilon$ characterizes the maximum change in the probability distribution of any defender due to changes in the states and actions of the other defenders. Parameter $\delta$ is set to $0$ in Algorithm \ref{algo:Stack}.} %Table \ref{table:robot} also gives the run time incurred when computing the stationary distribution using the Monte Carlo simulation and the solver time incurred to solve for the optimal policy of each agent. \textbf{Please ignore the numbers in this Table for now.}}
\label{table:security}
\end{table*}






\subsubsection{Simulation Results}


We use Algorithm~\ref{algo:Stack} to find a set of policies for the robots that maximizes their average reward. Table~\ref{table:robot} shows the simulation results of multi-robot control $\mathcal{M}$ under different sizes of grids $L$, number of agents $N$ and number of targets $B$. For each setting of $L$, $N$ and $B$ we vary the transition dependency parameter $\epsilon$ and record the average reward of Algorithm~\ref{algo:Stack} when parameter $\delta=0$. The parameters $K$, $\eta$, and $\beta$ are set to $1$, $0.75$ and $0.9$, respectively. Optimal values are calculated via evaluating the resulting $\mathcal{M}$ using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}. However, as the sizes of examples are increased, it incurs a heavy memory computation overhead to the system when using such an approach to solve $\mathcal{M}$. Specifically, for an example of $3$ robots trying to reach $1$ target in a $5 \times 5$ grid, it requires around 116 Gb of memory to compute the solution using such approach. Therefore, computing optimal value using such an approach is not computationally efficient for larger example sizes.

Overall we observe that our proposed approach provides average reward values closer to the optimal average reward values with more than $90\%$ of accuracy. We observe that the average reward values does not vary with $\epsilon$ dependency parameter when the number of agents are $2$. This is because when number of agents is small, they are able to find non overlapping paths to the target(s) in the grid and thus avoid collisions. When the number of agents increased we observe average reward increases with $\epsilon$ as it decreases the chances of agents colliding when trying to reach the target(s). Algorithm \ref{algo:Stack} takes about $30$s to calculate the policy for small-scale example with 2 agents, 1 target and $3\times 3$ grid , and takes around $1$ hour for larger-scale example with 3 agents, 1 target, and $4\times 4$ grid. More than $90\%$ of run time of Algorithm \ref{algo:Stack} is due to approximating the stationary distribution and average reward using Monte Carlo simulation.

% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Agents, Targets \\Number} & \thead{Grid\\ Size} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\eta=0.1$ & $\eta=0.5$ &$\eta = 0.9$ & $\eta=0.1$ & $\eta=0.5$ & $\eta=0.9$ & \thead{Avg. Run Time of\\ Algorithm \ref{algo:Stack}}\\
%     \hline
%   2, 1& $3 \times 3$ & 81 & 16 & 0.345 & 0.345 & 0.347 & 0.351& 0.351 & 0.351 & 26.47s\\
%   \hline
%   2, 2 & $3 \times 3$ & 81 & 16 & 0.441 & 0.440 & 0.439 & 0.443& 0.443 & 0.443 & 28.13s\\
%     \hline
%   2, 1 & $4 \times 4$ &256& 16  & 0.235 & 0.237 & 0.237 & 0.238  &0.238 & 0.238 & 56.00s\\
%     \hline
%     2, 2 & $4 \times 4$& 256 & 16 & 0.322 & 0.322 & 0.322 &0.328 & 0.328 & 0.328 & 75.33s\\
%     \hline
%     2, 1 & $5 \times 5$ & 625& 16 & 0.190 & 0.191 & 0.189 & 0.191 & 0.191 & 0.191 & 462.10s\\
%     \hline
%     3, 1 & $3 \times 3$ & 729 & 64 & 0.431  & 0.476 & 0.528 & 0.457 &  0.499 & 0.543  & 1754.84s \\
%     \hline
%     3, 1 & $4 \times 4$ & 4096  & 64 &  &  &  & &  & & \\
%     \hline
%     4, 1 & $2 \times 2$ & 256 & 256 & 0.621 & 0.660 & 0.752 & 0.634 &  0.670 & 0.761 & 586.64s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and average run time achieved using our proposed approach for different multi-agent robot control settings for three different dependency parameters ($\eta$ = $0.5$, $0.9$ and $0.1$). Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}. } 
% \label{table:robot}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%      \multicolumn{4}{|c|}{MMDP Setting} & \multicolumn{3}{|c|}{Average Reward} & \multicolumn{3}{|c|}{Optimal Value} & \\
%     \cline{1-10}
%     \thead{Defender, Adversary\\Number} & \thead{Location\\ Number} & \thead{State Space\\ Size} & \thead{Action Space\\ Size} &$\epsilon=0.1$ & $\epsilon=0.5$ &$\epsilon = 0.9$ & $\epsilon=0.1$ & $\epsilon=0.5$ & $\epsilon=0.9$ & \thead{Avg. Run Time \\of Algorithm \ref{algo:Stack}}\\
%     \hline
%   2,1& 3 & 27 & 27 & 0.563 & 0.563 & 0.563 & 0.563 & 0.563 & 0.563 & 10.7s\\
%   \hline
%   3,1 & 3 & 81 & 81 & 0.75 & 0.75 & 0.75 & 0.75& 0.75 & 0.75 & 105.5s\\
%     \hline
%   3,2 & 3 & 243 & 243  & 1.5 & 1.5 & 1.5 & 1.5  & 1.5 & 1.5 & 3092.31s\\
%     \hline
%     2,1 & 5 & 125 & 125 & 0.245 & 0.230 & 0.246 &0.46875 & 0.46875 & 0.46875 & 330.73s\\
%     \hline
%     3,1 & 5 & 625& 625 & 0.46 & 0.46 & 0.46 & 0.5625 &  0.5625& 0.5625 & 6803.3s\\
%     \hline
%     2,1 & 7 & 343& 343 & 0.29 & 0.29 & 0.29 & 0.4375 &  0.4375& 0.459 & 1080.66s\\
%     \hline
%     2,1 & 8 & 512& 512 & 0.18 & 0.18 & 0.18 & 0.428 & 0.428 & 0.428 & 4871.71s\\
%     \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Average reward and run time achieved using our proposed approach for different multi-agent security game settings with different dependency parameters $\epsilon$ ($\epsilon=0.1$, $0.5$ and $0.9$). The parameters $\eta$ and $\beta$ are set to $0.75$ and $0.5$, respectively. Parameters $c$ and $d$ are set as $c=d=1$. Optimal value for smaller problem sizes are calculated via solving the resulting MMDP using relative value iteration algorithm in \textit{Python MDP Toolbox} \cite{MDPtoolbox}.} %Table \ref{table:robot} also gives the run time incurred when computing the stationary distribution using the Monte Carlo simulation and the solver time incurred to solve for the optimal policy of each agent. \textbf{Please ignore the numbers in this Table for now.}}
% \label{table:security}
% \end{table*}


\subsection{Multi-Agent Security Game}
\subsubsection{Simulation Settings}
We implement our proposed approach on a security game \cite{tambe2011security} between multiple defenders and multiple adversaries among a finite set of locations $L$ as an evaluation. Each adversary and defender can pick some location to intrude and protect, respectively.

The security game is modeled by an MMDP $\mathcal{M}=(S,A,P,R)$, where $S=\times_iS_i\times_jS_j$ is the set of joint locations of the defenders and adversaries, with $S_i=L$ is the set of locations at which defender $i$ deploys its resource and $S_j=L$ is the set of locations where the adversary $j$ can intrude. The action of each defender and adversary is $A_i=A_j=L$. Thus the joint action space $A=\times_iA_i\times_jA_j$. For each defender $i$ and adversary $j$, we let
\begin{align*}
    &P_i(s_i, a_i,s_i') =\begin{cases}
    c&\mbox{ if } a_i=s_i', \not\exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \frac{1-c}{|L|}&\mbox{ if }a_i\neq s_i',\not\exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \epsilon c&\mbox{ if } a_i=s_i', \exists i'\neq i \text{ s.t. }a_{i}=a_{i'}\\
    \frac{1-\epsilon c}{|L|}&\mbox{ if } a_i\neq s_i', \exists i'\neq i \text{ s.t. }a_{i}=a_{i'}
    \end{cases}\\
    &P_j(s_j, a_j,s_j') =\begin{cases}
    d&\mbox{ if } a_j=s_j', \not\exists i \text{ s.t. }a_{i}=a_{j'}\\
    \frac{1-d}{|L|}&\mbox{ if }a_j\neq s_j', \not\exists i \text{ s.t. }a_{i}=a_{j'}\\
    \beta d&\mbox{ if } a_j=s_j', \exists i \text{ s.t. }a_{i}=a_{j'}\\
    \frac{1-\beta d}{|L|}&\mbox{ if } a_j\neq s_j',\exists i \text{ s.t. }a_{i}=a_{j'}
    \end{cases}
\end{align*}
Here parameters $c,d\in[0,1]$ capture the transition uncertainties \cite{jiang2013game}, parameter $\epsilon\in[0,1]$ captures the transition dependency between the defenders, and $\beta\in[0,1]$ captures the adversary's reaction to the defenders' actions. Let $s=\times_is_i\times_js_j$ and $s'=\times_is'_i\times_js'_j$ be two joint locations. Then $P(s,a,s')=\prod_{i,j}P_i(s_i,a_i,s_i')P_j(s_j,a_j,s_j')$, where $a=\times_is_i\times_js_j$. We define the reward function $R(s,a)$ for each $s\in S$ and $a\in A$ as $R(s,a)=\sum_{s'\in S}r(s,a,s')P(s,a,s')$, where $r(s,a,s')=\sum_{l\in L}(1-(1-\eta)^{k_l})x_l$, where $\eta\in(0,1]$ is the effectiveness parameter, $k$ and $x$ are the number of defenders and adversaries that are in location $l$ corresponding to $s'$, respectively.

% Given the current  location $s$, each defender $i$ computes its policy $\pi_i:S\mapsto L$ to determine the next location where its resource will be deployed. Each adversary $j$ determines its next location by following policy $\tau_j:S\mapsto L$. We assume that the policy of each adversary $j$ is known to the defenders. 

\subsubsection{Simulation Results}

In the following, we show our simulation results on multi-agent security game. We implement our proposed approach under various MMDP settings by varying the number of defenders, adversaries, and locations. For each MMDP setting, we vary the value of transition dependency parameter $\epsilon$, while fixing the other parameters. In particular, we fix the transition parameters for the defender and adversary as $c=d=1$. The transition dependency parameter for the adversary is $\beta=0.5$. The reward effectiveness parameter is set as $\eta=0.75$. We approximate the stationary distribution in \eqref{eq:TI-MDP-P} and \eqref{eq:TI-MDP-R} using Monte Carlo simulation. We test our proposed approach using 7 MMDP settings with one trial each, and detail the average reward of Algorithm \ref{algo:Stack} under each setting in Table \ref{table:security}.

We observe that when the number of locations is no less than the number of defenders, the policy returned by Algorithm \ref{algo:Stack} ensures minimum transition dependency between the defenders (e.g., 2nd - 4th row in Table \ref{table:security}). Therefore, the average reward does not vary when changing the value of $\epsilon$. We compare our proposed approach with the relative value iteration method over the joint state and action space. We note that our proposed approach recovers more than $90\%$ optimal average reward for small- and medium-scale problems, and incurs bounded performance loss for large scale problems (Theorem \ref{theorem:optimality}). By increasing the number of defenders and adversaries, the size of MMDP increases exponentially. Algorithm \ref{algo:Stack} takes about $10$s to compute the policy for small-scale example with 2 defenders, 1 adversary, and 3 locations, and about $80$ minutes for large-scale example with 2 defenders, 1 adversary, and $8$ locations. More than $90\%$ run time of Algorithm \ref{algo:Stack} is due to approximating the stationary distribution and average reward by simulations. %Although our proposed approach is slower compared with jointly optimizing over the original MDP, our approach is capable of handling problems of large scale that is intractable for the original MDP. 
% \textbf{2D1A7L optimal value runtime: 343.1s}
% \textbf{2D1A8L optimal value runtime: 1359.22s}

